Sim2Real Transfer for Audio-Visual Navigation with Frequency-Adaptive Acoustic Field Prediction

Sim2real transfer has received increasing attention lately due to the success of learning robotic tasks in simulation end-to-end. While there has been a lot of progress in transferring vision-based navigation policies, the existing sim2real strategy for audio-visual navigation performs data augmentation empirically without measuring the acoustic gap. The sound differs from light in that it spans across much wider frequencies and thus requires a different solution for sim2real. We propose the first treatment of sim2real for audio-visual navigation by disentangling it into acoustic field prediction (AFP) and waypoint navigation. We first validate our design choice in the SoundSpaces simulator and show improvement on the Continuous AudioGoal navigation benchmark. We then collect real-world data to measure the spectral difference between the simulation and the real world by training AFP models that only take a specific frequency subband as input. We further propose a frequency-adaptive strategy that intelligently selects the best frequency band for prediction based on both the measured spectral difference and the energy distribution of the received audio, which improves the performance on the real data. Lastly, we build a real robot platform and show that the transferred policy can successfully navigate to sounding objects. This work demonstrates the potential of building intelligent agents that can see, hear, and act entirely from simulation, and transferring them to the real world.

==> task.tex <==
\section{Background and Problem formulation}
\label{sec:task_formulation}

In this chapter, we outline several key topics that enhance the understanding of our research. Initially, we introduce the AudioGoal navigation task (Section \ref{sec:audio_nav_task}), which forms the basis of our second experiment (Section \ref{sec:exp_audiogoal_nav}). Subsequently, we discuss SoundSpaces 2.0 (Section \ref{sec:soundspaces2.0}), the simulation platform utilized for creating acoustic fields in our study. Finally, we elaborate on our specific definition of an acoustic field (Section \ref{sec:acoustic_field_def}).

\section{The Continuous AudioGoal Navigation Task}
\label{sec:audio_nav_task}
The AudioGoal navigation task (see Figure \ref{fig:audio_nav_task}) aims to test the navigation ability of the agent to find a particular sound source. Each test instance is called an episode. Each episode contains the starting position and rotation for the agent, and the location of the audio goal. The audio goal consists of a periodic, never-ending, invisible telephone sound, consistent with the methods used in previous studies~\cite{soundspaces_challenge, chen_soundspaces_2020, chen22soundspaces2}. The sound we chose for all experiments is a copyright-free telephone sound from \href{http://www.freesound.org}{freesound.org} and it is identical across all episodes. The sound, containing a one-second period, is located on the same floor as the starting position of the agent. At each time step, the agent can turn left, turn right, move forward, or stop. The agent can rotate at a 15-degree angle and move forward by 0.25 meters. If the agent issues a stop command within a 1-meter radius of the goal, the episode is considered successful; otherwise, it is considered a failure. In each episode, the agent also has a maximum of 500 time steps. The experiment simulates a scenario where the agent has to track a particular sound source such as a baby crying, telephone ringing, or alarm sounding. We assume there are no other sounds in the environment besides the sound source, following the setup from previous work~\cite{soundspaces_challenge,chen22soundspaces2, gan2020look,chen_avwan_2021}.

\begin{figure}[tb]
    \centering
    \includegraphics[width=0.4\textwidth,keepaspectratio]{audio_nav_task.png}
    \caption{An illustration of the AudioGoal navigation task. The agent is tasked to find the source of the periodic sound while minimizing the distance of the path traveled.}
    \label{fig:audio_nav_task}
\end{figure}

\section{SoundSpaces 2.0}
\label{sec:soundspaces2.0}
SoundSpaces~\cite{chen_soundspaces_2020}, initially introduced by Chen et al. in 2020, is a groundbreaking audio-visual simulation platform specifically designed for the training and evaluation of embodied AI agents. One of the key features of the original SoundSpaces is its pre-calculation of Room Impulse Response (RIR). This pre-calculation entails capturing the acoustic properties of various rooms in advance, thus enabling the simulation of sound within those environments. However, this approach allows only for discrete movement within the simulation. The agents can navigate from one pre-defined point to another, but cannot move continuously. This discrete movement model, while effective for certain types of simulations, does not fully replicate the fluid and dynamic nature of real-world navigation, where sound and movement are continuous and interdependent.

In response to this limitation, Chen et al. released SoundSpaces 2.0~\cite{chen22soundspaces2} in 2022. This updated version significantly enhances the platform by adding support for continuous navigation settings, aligning it more closely with real-world scenarios. SoundSpaces 2.0 can accurately model complex audio behaviors like echoes, reverberation, and absorption in any physical space, and it does so on the fly. This dynamic audio processing allows for a more realistic simulation experience, where the acoustic environment responds in real time to the continuous movement of AI agents.

However, the sophistication of SoundSpaces 2.0, particularly its real-time audio processing capability, increases the computational load. This makes the simulation process more resource-intensive, posing challenges for online reinforcement learning by complicating both the training and testing phases due to higher computational and time requirements.

Furthermore, SoundSpaces 2.0 maintains compatibility with arbitrary 3D scene datasets, such as Gibson~\cite{xia2018gibson}, MatterPort3D~\cite{Matterport3D}, and Replica~\cite{straub2019replica}. This compatibility enhances the versatility of the platform, allowing researchers to simulate a wide range of scenarios and environments, thereby providing rich and varied contexts for training and testing AI agents.

\subsection{Sim2real AudioGoal Navigation}
\vspace{2in}


